Energy dependence of $\phi$(1020) meson production in nucleus-nucleus collisions at the CERN SPS

This paper presents preliminary results from the NA61/SHINE experiment on $\phi$ meson production in central Ar+Sc collisions at beam momenta of 150$A$, 75$A$, and 40$A$ GeV/$c$ (corresponding to $\sqrt{s_{NN}}$ = 16.8, 11.9, and 8.8 GeV, respectively). These results include double differential distributions in rapidity ($y$) and transverse momentum ($p_T$), as well as $p_T$-integrated rapidity distributions and total $\phi$ yields. Additionally, the widths of the rapidity distributions of $\phi$ and $\phi/\pi$ yield ratios are compared to those from Pb+Pb and \pp reactions. Notably, this work represents the first-ever measurements of $\phi$ production in a mid-sized system at SPS energies.

==> numbers/ArSc150_rmsDoubleGauss.tex <==
0.994 \pm 0.020 \pm 0.018


==> numbers/ArSc150_totalYield.tex <==
1148 \pm 17 \pm 21


==> numbers/ArSc40_rmsDoubleGauss.tex <==
0.703 \pm 0.016 \pm 0.021


==> numbers/ArSc40_totalYield.tex <==
438 \pm 12 \pm 22


==> numbers/ArSc75_rmsDoubleGauss.tex <==
0.866 \pm 0.013 \pm 0.010


==> numbers/ArSc75_totalYield.tex <==
707 \pm 11 \pm 14

